Effects of charging and discharging capabilities on trade-offs between model accuracy and computational efficiency in pumped thermal electricity storage

The increasing need for energy storage solutions to balance variable renewable energy sources has highlighted the potential of Pumped Thermal Electricity Storage (PTES). In this paper, we investigate the trade-offs between model accuracy and computational efficiency in PTES systems. We evaluate a range of PTES models, from physically detailed to simplified variants, focusing on their non-linear charging and discharging capabilities. Our results show that while detailed models provide the most accurate representation of PTES operation by considering mass flow rate ($\dot{m}$) and state of charge (SoC) dependencies, they come at the cost of increased computational complexity. In contrast, simplified models tend to produce overly optimistic predictions by disregarding capability constraints. Other approximated model variants offer a practical compromise, balancing computational efficiency with acceptable accuracy. In particular, models that disregard $\dot{m}$-dependency and approximate nonlinear SoC-dependency with a piecewise linear function achieve similar accuracy to more detailed models but with significantly faster computation times. Our findings offer guidance to modelers in selecting the appropriate PTES representation for their investment models.

==> tex/00_Nomenclature.tex <==
\begin{table*}
\begin{framed}

\nomenclature[A]{CAISO}{California Independent System Operator}
\nomenclature[A]{CAPEX}{Capital Expenditure}
\nomenclature[A]{CEM}{Capacity expansion model}
\nomenclature[A]{ECDF}{Empirical Cumulative Density Function}
\nomenclature[A]{ERCOT}{Electric Reliability Council of Texas}
\nomenclature[A]{ISO}{Independent System Operator}
\nomenclature[A]{ISONE}{Independent System Operator New England}
\nomenclature[A]{FoM}{Figure of merit}
\nomenclature[A]{LDES}{Long-duration energy storage}
\nomenclature[A]{MILP}{Mixed-integer linear programming}
\nomenclature[A]{MISO}{Midcontinent Independent System Operator}
\nomenclature[A]{NYISO}{New York Independent System Operator}
\nomenclature[A]{OPEX}{Operating expense}
\nomenclature[A]{PJM}{Pennsylvania-New Jersey-Maryland}
\nomenclature[A]{PTES}{Pumped-thermal electricity storage}
\nomenclature[A]{RMSD}{Root-mean-square deviation}
\nomenclature[A]{RTO}{Regional Transmission Organization}
\nomenclature[A]{SoC}{State of charge}
\nomenclature[A]{SPP}{Southwest Power Pool}
\nomenclature[A]{TDR}{Time-domain reduction}
\nomenclature[A]{VRE}{Variable renewable energy}

\nomenclature[I]{\(h\)}{Hour}

\nomenclature[V]{\(P\)}{Total profit [\$]}
\nomenclature[V]{\(W\)}{Charging or discharing power [kW]}
\nomenclature[V]{\(\overline{W}\)}{Nominal charging or discharing power [kW]}
\nomenclature[V]{\(c\)}{Electricity price [\$/kW]}
\nomenclature[V]{\(\dot{m}\)}{Mass flow rate [kg/s]}
\nomenclature[V]{\(\overline{\dot{m}}\)}{Nominal mass flow rate [kg/s]}
\nomenclature[V]{\(p\)}{Part-load level [-]}
\nomenclature[V]{\(c_p\)}{Isobaric specific heat capacity [kJ/kg/K]}
\nomenclature[V]{\(T\)}{Temperature [K]}
\nomenclature[V]{\(\alpha\)}{Coefficient of performance [-]}
\nomenclature[V]{\(Q\)}{Heat flow rate [kW]}
\nomenclature[V]{\(\overline{Q}\)}{Nominal heat flow rate [kW]}
\nomenclature[V]{\(\eta\)}{Capability function [-]}

\begin{footnotesize}
\printnomenclature
\end{footnotesize}

\end{framed}
\end{table*}
